Galactic Winds and Extended Lya Emission from the Host Galaxies of High Column Density QSO Absorption Systems

We present 3D resonant radiative transfer simulations of the spatial and spectral diffusion of the Lya radiation from a central source in the host galaxies of high column density absorption systems at z ~ 3. The radiative transfer simulations are based on a suite of cosmological galaxy formation simulations that reproduce a wide range of observed properties of damped Lya absorption systems. The Lya emission is predicted to be spatially extended up to several arcsec, and the spectral width of the Lya emission is broadened to several hundred (in some case more than thousand) km/s. The distribution and the dynamical state of the gas in the simulated galaxies is complex, the latter with significant contributions from rotation and both in- and out-flows. The emerging Lya radiation extends to gas with column densities of N_HI ~ 10^{18} cm^{-2} and its spectral shape varies strongly with viewing angle. The strong dependence on the central \hi column density and the HI velocity field suggests that the Lya emission will also vary strongly with time on timescales of a few dynamical times of the central region. Such variations with time should be especially pronounced at times where the host galaxy undergoes a major merger and/or starburst. Depending on the pre-dominance of in- or out-flow along a given sightline and the central column density, the spectra show prominent blue peaks, red peaks or double-peaked profiles. Both spatial distribution and spectral shape are very sensitive to details of the galactic wind implementation. Stronger galactic winds result in more spatially extended Lya emission and - somewhat counterintuitively - a narrower spectral distribution.

==> momentum_grid0_Nim011.eps.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{Nim011.eps}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           29-Nov-2010 19:45:43
% eps bounding box:     15 cm x 12.5 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s04}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}y [arcsec]\end{tabular}}%
\psfrag{s05}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}z [arcsec]\end{tabular}}%
\psfrag{s06}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Viewpoint: x = -$\infty$\end{tabular}}%
\psfrag{s09}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}log N$_{\textrm{HI}}$   [cm$^{-2}$]\end{tabular}}%
%
% xticklabels:
\psfrag{x01}[t][t]{-8}%
\psfrag{x02}[t][t]{-6}%
\psfrag{x03}[t][t]{-4}%
\psfrag{x04}[t][t]{-2}%
\psfrag{x05}[t][t]{0}%
\psfrag{x06}[t][t]{2}%
\psfrag{x07}[t][t]{4}%
\psfrag{x08}[t][t]{6}%
\psfrag{x09}[t][t]{8}%
%
% yticklabels:
\psfrag{v01}[l][l]{13}%
\psfrag{v02}[l][l]{14}%
\psfrag{v03}[l][l]{15}%
\psfrag{v04}[l][l]{16}%
\psfrag{v05}[l][l]{17}%
\psfrag{v06}[l][l]{18}%
\psfrag{v07}[l][l]{19}%
\psfrag{v08}[l][l]{20}%
\psfrag{v09}[l][l]{21}%
\psfrag{v10}[l][l]{22}%
\psfrag{v11}[l][l]{23}%
\psfrag{v12}[r][r]{-8}%
\psfrag{v13}[r][r]{-6}%
\psfrag{v14}[r][r]{-4}%
\psfrag{v15}[r][r]{-2}%
\psfrag{v16}[r][r]{0}%
\psfrag{v17}[r][r]{2}%
\psfrag{v18}[r][r]{4}%
\psfrag{v19}[r][r]{6}%
\psfrag{v20}[r][r]{8}%
%
% Figure:
\includegraphics[width=\textwidth]{momentum_grid0_Nim011.eps.eps}
\end{psfrags}%
%
% End Nim011.eps.tex


==> momentum_grid0_Sim011.eps.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{Sim011.eps}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           29-Nov-2010 19:45:49
% eps bounding box:     15 cm x 12.5 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s04}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}y [arcsec]\end{tabular}}%
\psfrag{s05}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}z [arcsec]\end{tabular}}%
\psfrag{s09}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}log S   [erg/s/cm$^2$/arcsec$^2$]\end{tabular}}%
%
% xticklabels:
\psfrag{x01}[t][t]{-8}%
\psfrag{x02}[t][t]{-6}%
\psfrag{x03}[t][t]{-4}%
\psfrag{x04}[t][t]{-2}%
\psfrag{x05}[t][t]{0}%
\psfrag{x06}[t][t]{2}%
\psfrag{x07}[t][t]{4}%
\psfrag{x08}[t][t]{6}%
\psfrag{x09}[t][t]{8}%
%
% yticklabels:
\psfrag{v01}[l][l]{-23}%
\psfrag{v02}[l][l]{-22}%
\psfrag{v03}[l][l]{-21}%
\psfrag{v04}[l][l]{-20}%
\psfrag{v05}[l][l]{-19}%
\psfrag{v06}[l][l]{-18}%
\psfrag{v07}[l][l]{-17}%
\psfrag{v08}[l][l]{-16}%
\psfrag{v09}[l][l]{-15}%
\psfrag{v10}[r][r]{-8}%
\psfrag{v11}[r][r]{-6}%
\psfrag{v12}[r][r]{-4}%
\psfrag{v13}[r][r]{-2}%
\psfrag{v14}[r][r]{0}%
\psfrag{v15}[r][r]{2}%
\psfrag{v16}[r][r]{4}%
\psfrag{v17}[r][r]{6}%
\psfrag{v18}[r][r]{8}%
%
% Figure:
\includegraphics[width=\textwidth]{momentum_grid0_Sim011.eps.eps}
\end{psfrags}%
%
% End Sim011.eps.tex


==> momentum_grid0_Ssp0111v.eps.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{Ssp0111v.eps}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           29-Nov-2010 18:32:11
% eps bounding box:     14.2857 cm x 10.9751 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s04}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$v_{ph}$ [km/s]\end{tabular}}%
\psfrag{s05}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}y [arcsec]\end{tabular}}%
\psfrag{s09}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}log S$_{\lambda}$ [erg/s/cm$^2$/arcsec$^2$/\AA]\end{tabular}}%
%
% xticklabels:
\psfrag{x01}[t][t]{-2000}%
\psfrag{x02}[t][t]{-1000}%
\psfrag{x03}[t][t]{0}%
\psfrag{x04}[t][t]{1000}%
\psfrag{x05}[t][t]{2000}%
%
% yticklabels:
\psfrag{v01}[l][l]{-24}%
\psfrag{v02}[l][l]{-23}%
\psfrag{v03}[l][l]{-22}%
\psfrag{v04}[l][l]{-21}%
\psfrag{v05}[l][l]{-20}%
\psfrag{v06}[l][l]{-19}%
\psfrag{v07}[l][l]{-18}%
\psfrag{v08}[l][l]{-17}%
\psfrag{v09}[r][r]{-8}%
\psfrag{v10}[r][r]{-6}%
\psfrag{v11}[r][r]{-4}%
\psfrag{v12}[r][r]{-2}%
\psfrag{v13}[r][r]{0}%
\psfrag{v14}[r][r]{2}%
\psfrag{v15}[r][r]{4}%
\psfrag{v16}[r][r]{6}%
\psfrag{v17}[r][r]{8}%
%
% Figure:
\includegraphics[width=\textwidth]{momentum_grid0_Ssp0111v.eps.eps}
\end{psfrags}%
%
% End Ssp0111v.eps.tex


==> momentum_grid0_Ssp0112v.eps.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{Ssp0112v.eps}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           29-Nov-2010 18:32:15
% eps bounding box:     14.2857 cm x 10.9751 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s04}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$v_{ph}$ [km/s]\end{tabular}}%
\psfrag{s05}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}z [arcsec]\end{tabular}}%
\psfrag{s09}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}log S$_{\lambda}$ [erg/s/cm$^2$/arcsec$^2$/\AA]\end{tabular}}%
%
% xticklabels:
\psfrag{x01}[t][t]{-2000}%
\psfrag{x02}[t][t]{-1000}%
\psfrag{x03}[t][t]{0}%
\psfrag{x04}[t][t]{1000}%
\psfrag{x05}[t][t]{2000}%
%
% yticklabels:
\psfrag{v01}[l][l]{-24}%
\psfrag{v02}[l][l]{-23}%
\psfrag{v03}[l][l]{-22}%
\psfrag{v04}[l][l]{-21}%
\psfrag{v05}[l][l]{-20}%
\psfrag{v06}[l][l]{-19}%
\psfrag{v07}[l][l]{-18}%
\psfrag{v08}[l][l]{-17}%
\psfrag{v09}[r][r]{-8}%
\psfrag{v10}[r][r]{-6}%
\psfrag{v11}[r][r]{-4}%
\psfrag{v12}[r][r]{-2}%
\psfrag{v13}[r][r]{0}%
\psfrag{v14}[r][r]{2}%
\psfrag{v15}[r][r]{4}%
\psfrag{v16}[r][r]{6}%
\psfrag{v17}[r][r]{8}%
%
% Figure:
\includegraphics[width=\textwidth]{momentum_grid0_Ssp0112v.eps.eps}
\end{psfrags}%
%
% End Ssp0112v.eps.tex


==> momentum_grid4_Nim411.eps.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{Nim411.eps}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           29-Nov-2010 19:47:21
% eps bounding box:     15 cm x 12.5 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s04}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}y [arcsec]\end{tabular}}%
\psfrag{s05}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}z [arcsec]\end{tabular}}%
\psfrag{s06}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Viewpoint: x = -$\infty$\end{tabular}}%
\psfrag{s09}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}log N$_{\textrm{HI}}$   [cm$^{-2}$]\end{tabular}}%
%
% xticklabels:
\psfrag{x01}[t][t]{-4}%
\psfrag{x02}[t][t]{-3}%
\psfrag{x03}[t][t]{-2}%
\psfrag{x04}[t][t]{-1}%
\psfrag{x05}[t][t]{0}%
\psfrag{x06}[t][t]{1}%
\psfrag{x07}[t][t]{2}%
\psfrag{x08}[t][t]{3}%
\psfrag{x09}[t][t]{4}%
%
% yticklabels:
\psfrag{v01}[l][l]{13}%
\psfrag{v02}[l][l]{14}%
\psfrag{v03}[l][l]{15}%
\psfrag{v04}[l][l]{16}%
\psfrag{v05}[l][l]{17}%
\psfrag{v06}[l][l]{18}%
\psfrag{v07}[l][l]{19}%
\psfrag{v08}[l][l]{20}%
\psfrag{v09}[l][l]{21}%
\psfrag{v10}[l][l]{22}%
\psfrag{v11}[r][r]{-4}%
\psfrag{v12}[r][r]{-3}%
\psfrag{v13}[r][r]{-2}%
\psfrag{v14}[r][r]{-1}%
\psfrag{v15}[r][r]{0}%
\psfrag{v16}[r][r]{1}%
\psfrag{v17}[r][r]{2}%
\psfrag{v18}[r][r]{3}%
\psfrag{v19}[r][r]{4}%
%
% Figure:
\includegraphics[width=\textwidth]{momentum_grid4_Nim411.eps.eps}
\end{psfrags}%
%
% End Nim411.eps.tex


==> momentum_grid4_Sim411.eps.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{Sim411.eps}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           29-Nov-2010 19:47:26
% eps bounding box:     15 cm x 12.5 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s04}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}y [arcsec]\end{tabular}}%
\psfrag{s05}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}z [arcsec]\end{tabular}}%
\psfrag{s09}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}log S   [erg/s/cm$^2$/arcsec$^2$]\end{tabular}}%
%
% xticklabels:
\psfrag{x01}[t][t]{-4}%
\psfrag{x02}[t][t]{-3}%
\psfrag{x03}[t][t]{-2}%
\psfrag{x04}[t][t]{-1}%
\psfrag{x05}[t][t]{0}%
\psfrag{x06}[t][t]{1}%
\psfrag{x07}[t][t]{2}%
\psfrag{x08}[t][t]{3}%
\psfrag{x09}[t][t]{4}%
%
% yticklabels:
\psfrag{v01}[l][l]{-23}%
\psfrag{v02}[l][l]{-22}%
\psfrag{v03}[l][l]{-21}%
\psfrag{v04}[l][l]{-20}%
\psfrag{v05}[l][l]{-19}%
\psfrag{v06}[l][l]{-18}%
\psfrag{v07}[l][l]{-17}%
\psfrag{v08}[l][l]{-16}%
\psfrag{v09}[r][r]{-4}%
\psfrag{v10}[r][r]{-3}%
\psfrag{v11}[r][r]{-2}%
\psfrag{v12}[r][r]{-1}%
\psfrag{v13}[r][r]{0}%
\psfrag{v14}[r][r]{1}%
\psfrag{v15}[r][r]{2}%
\psfrag{v16}[r][r]{3}%
\psfrag{v17}[r][r]{4}%
%
% Figure:
\includegraphics[width=\textwidth]{momentum_grid4_Sim411.eps.eps}
\end{psfrags}%
%
% End Sim411.eps.tex


==> momentum_grid4_Ssp4111v.eps.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{Ssp4111v.eps}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           29-Nov-2010 18:37:42
% eps bounding box:     14.2857 cm x 10.9751 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s04}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$v_{ph}$ [km/s]\end{tabular}}%
\psfrag{s05}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}y [arcsec]\end{tabular}}%
\psfrag{s09}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}log S$_{\lambda}$ [erg/s/cm$^2$/arcsec$^2$/\AA]\end{tabular}}%
%
% xticklabels:
\psfrag{x01}[t][t]{-1000}%
\psfrag{x02}[t][t]{-500}%
\psfrag{x03}[t][t]{0}%
\psfrag{x04}[t][t]{500}%
\psfrag{x05}[t][t]{1000}%
%
% yticklabels:
\psfrag{v01}[l][l]{-25}%
\psfrag{v02}[l][l]{-24}%
\psfrag{v03}[l][l]{-23}%
\psfrag{v04}[l][l]{-22}%
\psfrag{v05}[l][l]{-21}%
\psfrag{v06}[l][l]{-20}%
\psfrag{v07}[l][l]{-19}%
\psfrag{v08}[l][l]{-18}%
\psfrag{v09}[r][r]{-4}%
\psfrag{v10}[r][r]{-3}%
\psfrag{v11}[r][r]{-2}%
\psfrag{v12}[r][r]{-1}%
\psfrag{v13}[r][r]{0}%
\psfrag{v14}[r][r]{1}%
\psfrag{v15}[r][r]{2}%
\psfrag{v16}[r][r]{3}%
\psfrag{v17}[r][r]{4}%
%
% Figure:
\includegraphics[width=\textwidth]{momentum_grid4_Ssp4111v.eps.eps}
\end{psfrags}%
%
% End Ssp4111v.eps.tex


==> momentum_grid4_Ssp4112v.eps.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{Ssp4112v.eps}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           29-Nov-2010 18:37:44
% eps bounding box:     14.2857 cm x 10.9751 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s04}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$v_{ph}$ [km/s]\end{tabular}}%
\psfrag{s05}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}z [arcsec]\end{tabular}}%
\psfrag{s09}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}log S$_{\lambda}$ [erg/s/cm$^2$/arcsec$^2$/\AA]\end{tabular}}%
%
% xticklabels:
\psfrag{x01}[t][t]{-1000}%
\psfrag{x02}[t][t]{-500}%
\psfrag{x03}[t][t]{0}%
\psfrag{x04}[t][t]{500}%
\psfrag{x05}[t][t]{1000}%
%
% yticklabels:
\psfrag{v01}[l][l]{-25}%
\psfrag{v02}[l][l]{-24}%
\psfrag{v03}[l][l]{-23}%
\psfrag{v04}[l][l]{-22}%
\psfrag{v05}[l][l]{-21}%
\psfrag{v06}[l][l]{-20}%
\psfrag{v07}[l][l]{-19}%
\psfrag{v08}[l][l]{-18}%
\psfrag{v09}[r][r]{-4}%
\psfrag{v10}[r][r]{-3}%
\psfrag{v11}[r][r]{-2}%
\psfrag{v12}[r][r]{-1}%
\psfrag{v13}[r][r]{0}%
\psfrag{v14}[r][r]{1}%
\psfrag{v15}[r][r]{2}%
\psfrag{v16}[r][r]{3}%
\psfrag{v17}[r][r]{4}%
%
% Figure:
\includegraphics[width=\textwidth]{momentum_grid4_Ssp4112v.eps.eps}
\end{psfrags}%
%
% End Ssp4112v.eps.tex


==> momentum_grid7_Nim711.eps.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{Nim711.eps}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           29-Nov-2010 19:48:06
% eps bounding box:     15 cm x 12.5 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s04}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}y [arcsec]\end{tabular}}%
\psfrag{s05}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}z [arcsec]\end{tabular}}%
\psfrag{s06}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Viewpoint: x = -$\infty$\end{tabular}}%
\psfrag{s09}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}log N$_{\textrm{HI}}$   [cm$^{-2}$]\end{tabular}}%
%
% xticklabels:
\psfrag{x01}[t][t]{-8}%
\psfrag{x02}[t][t]{-6}%
\psfrag{x03}[t][t]{-4}%
\psfrag{x04}[t][t]{-2}%
\psfrag{x05}[t][t]{0}%
\psfrag{x06}[t][t]{2}%
\psfrag{x07}[t][t]{4}%
\psfrag{x08}[t][t]{6}%
\psfrag{x09}[t][t]{8}%
%
% yticklabels:
\psfrag{v01}[l][l]{13}%
\psfrag{v02}[l][l]{14}%
\psfrag{v03}[l][l]{15}%
\psfrag{v04}[l][l]{16}%
\psfrag{v05}[l][l]{17}%
\psfrag{v06}[l][l]{18}%
\psfrag{v07}[l][l]{19}%
\psfrag{v08}[l][l]{20}%
\psfrag{v09}[l][l]{21}%
\psfrag{v10}[l][l]{22}%
\psfrag{v11}[l][l]{23}%
\psfrag{v12}[r][r]{-8}%
\psfrag{v13}[r][r]{-6}%
\psfrag{v14}[r][r]{-4}%
\psfrag{v15}[r][r]{-2}%
\psfrag{v16}[r][r]{0}%
\psfrag{v17}[r][r]{2}%
\psfrag{v18}[r][r]{4}%
\psfrag{v19}[r][r]{6}%
\psfrag{v20}[r][r]{8}%
%
% Figure:
\includegraphics[width=\textwidth]{momentum_grid7_Nim711.eps.eps}
\end{psfrags}%
%
% End Nim711.eps.tex


==> momentum_grid7_Nim712.eps.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{Nim712.eps}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           29-Nov-2010 19:48:07
% eps bounding box:     15 cm x 12.5 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s04}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}y [arcsec]\end{tabular}}%
\psfrag{s05}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}z [arcsec]\end{tabular}}%
\psfrag{s06}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Viewpoint: x = +$\infty$\end{tabular}}%
\psfrag{s09}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}log N$_{\textrm{HI}}$   [cm$^{-2}$]\end{tabular}}%
%
% xticklabels:
\psfrag{x01}[t][t]{-8}%
\psfrag{x02}[t][t]{-6}%
\psfrag{x03}[t][t]{-4}%
\psfrag{x04}[t][t]{-2}%
\psfrag{x05}[t][t]{0}%
\psfrag{x06}[t][t]{2}%
\psfrag{x07}[t][t]{4}%
\psfrag{x08}[t][t]{6}%
\psfrag{x09}[t][t]{8}%
%
% yticklabels:
\psfrag{v01}[l][l]{13}%
\psfrag{v02}[l][l]{14}%
\psfrag{v03}[l][l]{15}%
\psfrag{v04}[l][l]{16}%
\psfrag{v05}[l][l]{17}%
\psfrag{v06}[l][l]{18}%
\psfrag{v07}[l][l]{19}%
\psfrag{v08}[l][l]{20}%
\psfrag{v09}[l][l]{21}%
\psfrag{v10}[l][l]{22}%
\psfrag{v11}[l][l]{23}%
\psfrag{v12}[r][r]{-8}%
\psfrag{v13}[r][r]{-6}%
\psfrag{v14}[r][r]{-4}%
\psfrag{v15}[r][r]{-2}%
\psfrag{v16}[r][r]{0}%
\psfrag{v17}[r][r]{2}%
\psfrag{v18}[r][r]{4}%
\psfrag{v19}[r][r]{6}%
\psfrag{v20}[r][r]{8}%
%
% Figure:
\includegraphics[width=\textwidth]{momentum_grid7_Nim712.eps.eps}
\end{psfrags}%
%
% End Nim712.eps.tex


==> momentum_grid7_Sim711.eps.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{Sim711.eps}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           29-Nov-2010 19:48:12
% eps bounding box:     15 cm x 12.5 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s04}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}y [arcsec]\end{tabular}}%
\psfrag{s05}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}z [arcsec]\end{tabular}}%
\psfrag{s09}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}log S   [erg/s/cm$^2$/arcsec$^2$]\end{tabular}}%
%
% xticklabels:
\psfrag{x01}[t][t]{-8}%
\psfrag{x02}[t][t]{-6}%
\psfrag{x03}[t][t]{-4}%
\psfrag{x04}[t][t]{-2}%
\psfrag{x05}[t][t]{0}%
\psfrag{x06}[t][t]{2}%
\psfrag{x07}[t][t]{4}%
\psfrag{x08}[t][t]{6}%
\psfrag{x09}[t][t]{8}%
%
% yticklabels:
\psfrag{v01}[l][l]{-23}%
\psfrag{v02}[l][l]{-22}%
\psfrag{v03}[l][l]{-21}%
\psfrag{v04}[l][l]{-20}%
\psfrag{v05}[l][l]{-19}%
\psfrag{v06}[l][l]{-18}%
\psfrag{v07}[l][l]{-17}%
\psfrag{v08}[l][l]{-16}%
\psfrag{v09}[r][r]{-8}%
\psfrag{v10}[r][r]{-6}%
\psfrag{v11}[r][r]{-4}%
\psfrag{v12}[r][r]{-2}%
\psfrag{v13}[r][r]{0}%
\psfrag{v14}[r][r]{2}%
\psfrag{v15}[r][r]{4}%
\psfrag{v16}[r][r]{6}%
\psfrag{v17}[r][r]{8}%
%
% Figure:
\includegraphics[width=\textwidth]{momentum_grid7_Sim711.eps.eps}
\end{psfrags}%
%
% End Sim711.eps.tex


==> momentum_grid7_Sim712.eps.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{Sim712.eps}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           29-Nov-2010 19:48:13
% eps bounding box:     15 cm x 12.5 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s04}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}y [arcsec]\end{tabular}}%
\psfrag{s05}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}z [arcsec]\end{tabular}}%
\psfrag{s09}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}log S   [erg/s/cm$^2$/arcsec$^2$]\end{tabular}}%
%
% xticklabels:
\psfrag{x01}[t][t]{-8}%
\psfrag{x02}[t][t]{-6}%
\psfrag{x03}[t][t]{-4}%
\psfrag{x04}[t][t]{-2}%
\psfrag{x05}[t][t]{0}%
\psfrag{x06}[t][t]{2}%
\psfrag{x07}[t][t]{4}%
\psfrag{x08}[t][t]{6}%
\psfrag{x09}[t][t]{8}%
%
% yticklabels:
\psfrag{v01}[l][l]{-23}%
\psfrag{v02}[l][l]{-22}%
\psfrag{v03}[l][l]{-21}%
\psfrag{v04}[l][l]{-20}%
\psfrag{v05}[l][l]{-19}%
\psfrag{v06}[l][l]{-18}%
\psfrag{v07}[l][l]{-17}%
\psfrag{v08}[l][l]{-16}%
\psfrag{v09}[r][r]{-8}%
\psfrag{v10}[r][r]{-6}%
\psfrag{v11}[r][r]{-4}%
\psfrag{v12}[r][r]{-2}%
\psfrag{v13}[r][r]{0}%
\psfrag{v14}[r][r]{2}%
\psfrag{v15}[r][r]{4}%
\psfrag{v16}[r][r]{6}%
\psfrag{v17}[r][r]{8}%
%
% Figure:
\includegraphics[width=\textwidth]{momentum_grid7_Sim712.eps.eps}
\end{psfrags}%
%
% End Sim712.eps.tex


==> momentum_grid7_Ssp7111v.eps.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{Ssp7111v.eps}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           29-Nov-2010 18:39:55
% eps bounding box:     14.2857 cm x 10.9751 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s04}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$v_{ph}$ [km/s]\end{tabular}}%
\psfrag{s05}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}y [arcsec]\end{tabular}}%
\psfrag{s09}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}log S$_{\lambda}$ [erg/s/cm$^2$/arcsec$^2$/\AA]\end{tabular}}%
%
% xticklabels:
\psfrag{x01}[t][t]{-1500}%
\psfrag{x02}[t][t]{-1000}%
\psfrag{x03}[t][t]{-500}%
\psfrag{x04}[t][t]{0}%
\psfrag{x05}[t][t]{500}%
\psfrag{x06}[t][t]{1000}%
\psfrag{x07}[t][t]{1500}%
%
% yticklabels:
\psfrag{v01}[l][l]{-25}%
\psfrag{v02}[l][l]{-24}%
\psfrag{v03}[l][l]{-23}%
\psfrag{v04}[l][l]{-22}%
\psfrag{v05}[l][l]{-21}%
\psfrag{v06}[l][l]{-20}%
\psfrag{v07}[l][l]{-19}%
\psfrag{v08}[l][l]{-18}%
\psfrag{v09}[l][l]{-17}%
\psfrag{v10}[r][r]{-8}%
\psfrag{v11}[r][r]{-6}%
\psfrag{v12}[r][r]{-4}%
\psfrag{v13}[r][r]{-2}%
\psfrag{v14}[r][r]{0}%
\psfrag{v15}[r][r]{2}%
\psfrag{v16}[r][r]{4}%
\psfrag{v17}[r][r]{6}%
\psfrag{v18}[r][r]{8}%
%
% Figure:
\includegraphics[width=\textwidth]{momentum_grid7_Ssp7111v.eps.eps}
\end{psfrags}%
%
% End Ssp7111v.eps.tex


==> momentum_grid7_Ssp7112v.eps.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{Ssp7112v.eps}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           29-Nov-2010 18:39:59
% eps bounding box:     14.2857 cm x 10.9751 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s04}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$v_{ph}$ [km/s]\end{tabular}}%
\psfrag{s05}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}z [arcsec]\end{tabular}}%
\psfrag{s09}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}log S$_{\lambda}$ [erg/s/cm$^2$/arcsec$^2$/\AA]\end{tabular}}%
%
% xticklabels:
\psfrag{x01}[t][t]{-1500}%
\psfrag{x02}[t][t]{-1000}%
\psfrag{x03}[t][t]{-500}%
\psfrag{x04}[t][t]{0}%
\psfrag{x05}[t][t]{500}%
\psfrag{x06}[t][t]{1000}%
\psfrag{x07}[t][t]{1500}%
%
% yticklabels:
\psfrag{v01}[l][l]{-25}%
\psfrag{v02}[l][l]{-24}%
\psfrag{v03}[l][l]{-23}%
\psfrag{v04}[l][l]{-22}%
\psfrag{v05}[l][l]{-21}%
\psfrag{v06}[l][l]{-20}%
\psfrag{v07}[l][l]{-19}%
\psfrag{v08}[l][l]{-18}%
\psfrag{v09}[l][l]{-17}%
\psfrag{v10}[r][r]{-8}%
\psfrag{v11}[r][r]{-6}%
\psfrag{v12}[r][r]{-4}%
\psfrag{v13}[r][r]{-2}%
\psfrag{v14}[r][r]{0}%
\psfrag{v15}[r][r]{2}%
\psfrag{v16}[r][r]{4}%
\psfrag{v17}[r][r]{6}%
\psfrag{v18}[r][r]{8}%
%
% Figure:
\includegraphics[width=\textwidth]{momentum_grid7_Ssp7112v.eps.eps}
\end{psfrags}%
%
% End Ssp7112v.eps.tex


==> momentum_grid7_Ssp7121v.eps.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{Ssp7121v.eps}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           29-Nov-2010 18:40:02
% eps bounding box:     14.2857 cm x 10.9751 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s04}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$v_{ph}$ [km/s]\end{tabular}}%
\psfrag{s05}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}y [arcsec]\end{tabular}}%
\psfrag{s09}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}log S$_{\lambda}$ [erg/s/cm$^2$/arcsec$^2$/\AA]\end{tabular}}%
%
% xticklabels:
\psfrag{x01}[t][t]{-1500}%
\psfrag{x02}[t][t]{-1000}%
\psfrag{x03}[t][t]{-500}%
\psfrag{x04}[t][t]{0}%
\psfrag{x05}[t][t]{500}%
\psfrag{x06}[t][t]{1000}%
\psfrag{x07}[t][t]{1500}%
%
% yticklabels:
\psfrag{v01}[l][l]{-25}%
\psfrag{v02}[l][l]{-24}%
\psfrag{v03}[l][l]{-23}%
\psfrag{v04}[l][l]{-22}%
\psfrag{v05}[l][l]{-21}%
\psfrag{v06}[l][l]{-20}%
\psfrag{v07}[l][l]{-19}%
\psfrag{v08}[l][l]{-18}%
\psfrag{v09}[l][l]{-17}%
\psfrag{v10}[r][r]{-8}%
\psfrag{v11}[r][r]{-6}%
\psfrag{v12}[r][r]{-4}%
\psfrag{v13}[r][r]{-2}%
\psfrag{v14}[r][r]{0}%
\psfrag{v15}[r][r]{2}%
\psfrag{v16}[r][r]{4}%
\psfrag{v17}[r][r]{6}%
\psfrag{v18}[r][r]{8}%
%
% Figure:
\includegraphics[width=\textwidth]{momentum_grid7_Ssp7121v.eps.eps}
\end{psfrags}%
%
% End Ssp7121v.eps.tex


==> momentum_grid7_Ssp7122v.eps.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{Ssp7122v.eps}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           29-Nov-2010 18:40:05
% eps bounding box:     14.2857 cm x 10.9751 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s04}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$v_{ph}$ [km/s]\end{tabular}}%
\psfrag{s05}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}z [arcsec]\end{tabular}}%
\psfrag{s09}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}log S$_{\lambda}$ [erg/s/cm$^2$/arcsec$^2$/\AA]\end{tabular}}%
%
% xticklabels:
\psfrag{x01}[t][t]{-1500}%
\psfrag{x02}[t][t]{-1000}%
\psfrag{x03}[t][t]{-500}%
\psfrag{x04}[t][t]{0}%
\psfrag{x05}[t][t]{500}%
\psfrag{x06}[t][t]{1000}%
\psfrag{x07}[t][t]{1500}%
%
% yticklabels:
\psfrag{v01}[l][l]{-25}%
\psfrag{v02}[l][l]{-24}%
\psfrag{v03}[l][l]{-23}%
\psfrag{v04}[l][l]{-22}%
\psfrag{v05}[l][l]{-21}%
\psfrag{v06}[l][l]{-20}%
\psfrag{v07}[l][l]{-19}%
\psfrag{v08}[l][l]{-18}%
\psfrag{v09}[l][l]{-17}%
\psfrag{v10}[r][r]{-8}%
\psfrag{v11}[r][r]{-6}%
\psfrag{v12}[r][r]{-4}%
\psfrag{v13}[r][r]{-2}%
\psfrag{v14}[r][r]{0}%
\psfrag{v15}[r][r]{2}%
\psfrag{v16}[r][r]{4}%
\psfrag{v17}[r][r]{6}%
\psfrag{v18}[r][r]{8}%
%
% Figure:
\includegraphics[width=\textwidth]{momentum_grid7_Ssp7122v.eps.eps}
\end{psfrags}%
%
% End Ssp7122v.eps.tex


==> weak_grid0_Nim011.eps.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{Nim011.eps}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           29-Nov-2010 19:46:12
% eps bounding box:     15 cm x 12.5 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s04}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}y [arcsec]\end{tabular}}%
\psfrag{s05}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}z [arcsec]\end{tabular}}%
\psfrag{s06}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Viewpoint: x = -$\infty$\end{tabular}}%
\psfrag{s09}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}log N$_{\textrm{HI}}$   [cm$^{-2}$]\end{tabular}}%
%
% xticklabels:
\psfrag{x01}[t][t]{-8}%
\psfrag{x02}[t][t]{-6}%
\psfrag{x03}[t][t]{-4}%
\psfrag{x04}[t][t]{-2}%
\psfrag{x05}[t][t]{0}%
\psfrag{x06}[t][t]{2}%
\psfrag{x07}[t][t]{4}%
\psfrag{x08}[t][t]{6}%
\psfrag{x09}[t][t]{8}%
%
% yticklabels:
\psfrag{v01}[l][l]{13}%
\psfrag{v02}[l][l]{14}%
\psfrag{v03}[l][l]{15}%
\psfrag{v04}[l][l]{16}%
\psfrag{v05}[l][l]{17}%
\psfrag{v06}[l][l]{18}%
\psfrag{v07}[l][l]{19}%
\psfrag{v08}[l][l]{20}%
\psfrag{v09}[l][l]{21}%
\psfrag{v10}[l][l]{22}%
\psfrag{v11}[l][l]{23}%
\psfrag{v12}[r][r]{-8}%
\psfrag{v13}[r][r]{-6}%
\psfrag{v14}[r][r]{-4}%
\psfrag{v15}[r][r]{-2}%
\psfrag{v16}[r][r]{0}%
\psfrag{v17}[r][r]{2}%
\psfrag{v18}[r][r]{4}%
\psfrag{v19}[r][r]{6}%
\psfrag{v20}[r][r]{8}%
%
% Figure:
\includegraphics[width=\textwidth]{weak_grid0_Nim011.eps.eps}
\end{psfrags}%
%
% End Nim011.eps.tex


==> weak_grid0_Sim011.eps.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{Sim011.eps}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           29-Nov-2010 19:46:18
% eps bounding box:     15 cm x 12.5 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s04}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}y [arcsec]\end{tabular}}%
\psfrag{s05}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}z [arcsec]\end{tabular}}%
\psfrag{s09}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}log S   [erg/s/cm$^2$/arcsec$^2$]\end{tabular}}%
%
% xticklabels:
\psfrag{x01}[t][t]{-8}%
\psfrag{x02}[t][t]{-6}%
\psfrag{x03}[t][t]{-4}%
\psfrag{x04}[t][t]{-2}%
\psfrag{x05}[t][t]{0}%
\psfrag{x06}[t][t]{2}%
\psfrag{x07}[t][t]{4}%
\psfrag{x08}[t][t]{6}%
\psfrag{x09}[t][t]{8}%
%
% yticklabels:
\psfrag{v01}[l][l]{-23}%
\psfrag{v02}[l][l]{-22}%
\psfrag{v03}[l][l]{-21}%
\psfrag{v04}[l][l]{-20}%
\psfrag{v05}[l][l]{-19}%
\psfrag{v06}[l][l]{-18}%
\psfrag{v07}[l][l]{-17}%
\psfrag{v08}[l][l]{-16}%
\psfrag{v09}[l][l]{-15}%
\psfrag{v10}[r][r]{-8}%
\psfrag{v11}[r][r]{-6}%
\psfrag{v12}[r][r]{-4}%
\psfrag{v13}[r][r]{-2}%
\psfrag{v14}[r][r]{0}%
\psfrag{v15}[r][r]{2}%
\psfrag{v16}[r][r]{4}%
\psfrag{v17}[r][r]{6}%
\psfrag{v18}[r][r]{8}%
%
% Figure:
\includegraphics[width=\textwidth]{weak_grid0_Sim011.eps.eps}
\end{psfrags}%
%
% End Sim011.eps.tex


==> weak_grid0_Ssp0111v.eps.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{Ssp0111v.eps}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           29-Nov-2010 18:33:53
% eps bounding box:     14.2857 cm x 10.9751 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s04}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$v_{ph}$ [km/s]\end{tabular}}%
\psfrag{s05}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}y [arcsec]\end{tabular}}%
\psfrag{s09}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}log S$_{\lambda}$ [erg/s/cm$^2$/arcsec$^2$/\AA]\end{tabular}}%
%
% xticklabels:
\psfrag{x01}[t][t]{-5000}%
\psfrag{x02}[t][t]{0}%
\psfrag{x03}[t][t]{5000}%
%
% yticklabels:
\psfrag{v01}[l][l]{-24}%
\psfrag{v02}[l][l]{-23}%
\psfrag{v03}[l][l]{-22}%
\psfrag{v04}[l][l]{-21}%
\psfrag{v05}[l][l]{-20}%
\psfrag{v06}[l][l]{-19}%
\psfrag{v07}[l][l]{-18}%
\psfrag{v08}[l][l]{-17}%
\psfrag{v09}[r][r]{-8}%
\psfrag{v10}[r][r]{-6}%
\psfrag{v11}[r][r]{-4}%
\psfrag{v12}[r][r]{-2}%
\psfrag{v13}[r][r]{0}%
\psfrag{v14}[r][r]{2}%
\psfrag{v15}[r][r]{4}%
\psfrag{v16}[r][r]{6}%
\psfrag{v17}[r][r]{8}%
%
% Figure:
\includegraphics[width=\textwidth]{weak_grid0_Ssp0111v.eps.eps}
\end{psfrags}%
%
% End Ssp0111v.eps.tex


==> weak_grid0_Ssp0112v.eps.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{Ssp0112v.eps}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           29-Nov-2010 18:33:57
% eps bounding box:     14.2857 cm x 10.9751 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s04}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$v_{ph}$ [km/s]\end{tabular}}%
\psfrag{s05}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}z [arcsec]\end{tabular}}%
\psfrag{s09}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}log S$_{\lambda}$ [erg/s/cm$^2$/arcsec$^2$/\AA]\end{tabular}}%
%
% xticklabels:
\psfrag{x01}[t][t]{-5000}%
\psfrag{x02}[t][t]{0}%
\psfrag{x03}[t][t]{5000}%
%
% yticklabels:
\psfrag{v01}[l][l]{-24}%
\psfrag{v02}[l][l]{-23}%
\psfrag{v03}[l][l]{-22}%
\psfrag{v04}[l][l]{-21}%
\psfrag{v05}[l][l]{-20}%
\psfrag{v06}[l][l]{-19}%
\psfrag{v07}[l][l]{-18}%
\psfrag{v08}[l][l]{-17}%
\psfrag{v09}[r][r]{-8}%
\psfrag{v10}[r][r]{-6}%
\psfrag{v11}[r][r]{-4}%
\psfrag{v12}[r][r]{-2}%
\psfrag{v13}[r][r]{0}%
\psfrag{v14}[r][r]{2}%
\psfrag{v15}[r][r]{4}%
\psfrag{v16}[r][r]{6}%
\psfrag{v17}[r][r]{8}%
%
% Figure:
\includegraphics[width=\textwidth]{weak_grid0_Ssp0112v.eps.eps}
\end{psfrags}%
%
% End Ssp0112v.eps.tex


==> weak_grid4_Nim411.eps.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{Nim411.eps}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           29-Nov-2010 19:47:43
% eps bounding box:     15 cm x 12.5 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s04}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}y [arcsec]\end{tabular}}%
\psfrag{s05}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}z [arcsec]\end{tabular}}%
\psfrag{s06}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Viewpoint: x = -$\infty$\end{tabular}}%
\psfrag{s09}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}log N$_{\textrm{HI}}$   [cm$^{-2}$]\end{tabular}}%
%
% xticklabels:
\psfrag{x01}[t][t]{-4}%
\psfrag{x02}[t][t]{-3}%
\psfrag{x03}[t][t]{-2}%
\psfrag{x04}[t][t]{-1}%
\psfrag{x05}[t][t]{0}%
\psfrag{x06}[t][t]{1}%
\psfrag{x07}[t][t]{2}%
\psfrag{x08}[t][t]{3}%
\psfrag{x09}[t][t]{4}%
%
% yticklabels:
\psfrag{v01}[l][l]{13}%
\psfrag{v02}[l][l]{14}%
\psfrag{v03}[l][l]{15}%
\psfrag{v04}[l][l]{16}%
\psfrag{v05}[l][l]{17}%
\psfrag{v06}[l][l]{18}%
\psfrag{v07}[l][l]{19}%
\psfrag{v08}[l][l]{20}%
\psfrag{v09}[l][l]{21}%
\psfrag{v10}[l][l]{22}%
\psfrag{v11}[r][r]{-4}%
\psfrag{v12}[r][r]{-3}%
\psfrag{v13}[r][r]{-2}%
\psfrag{v14}[r][r]{-1}%
\psfrag{v15}[r][r]{0}%
\psfrag{v16}[r][r]{1}%
\psfrag{v17}[r][r]{2}%
\psfrag{v18}[r][r]{3}%
\psfrag{v19}[r][r]{4}%
%
% Figure:
\includegraphics[width=\textwidth]{weak_grid4_Nim411.eps.eps}
\end{psfrags}%
%
% End Nim411.eps.tex


==> weak_grid4_Sim411.eps.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{Sim411.eps}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           29-Nov-2010 19:47:49
% eps bounding box:     15 cm x 12.5 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s04}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}y [arcsec]\end{tabular}}%
\psfrag{s05}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}z [arcsec]\end{tabular}}%
\psfrag{s09}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}log S   [erg/s/cm$^2$/arcsec$^2$]\end{tabular}}%
%
% xticklabels:
\psfrag{x01}[t][t]{-4}%
\psfrag{x02}[t][t]{-3}%
\psfrag{x03}[t][t]{-2}%
\psfrag{x04}[t][t]{-1}%
\psfrag{x05}[t][t]{0}%
\psfrag{x06}[t][t]{1}%
\psfrag{x07}[t][t]{2}%
\psfrag{x08}[t][t]{3}%
\psfrag{x09}[t][t]{4}%
%
% yticklabels:
\psfrag{v01}[l][l]{-23}%
\psfrag{v02}[l][l]{-22}%
\psfrag{v03}[l][l]{-21}%
\psfrag{v04}[l][l]{-20}%
\psfrag{v05}[l][l]{-19}%
\psfrag{v06}[l][l]{-18}%
\psfrag{v07}[l][l]{-17}%
\psfrag{v08}[l][l]{-16}%
\psfrag{v09}[r][r]{-4}%
\psfrag{v10}[r][r]{-3}%
\psfrag{v11}[r][r]{-2}%
\psfrag{v12}[r][r]{-1}%
\psfrag{v13}[r][r]{0}%
\psfrag{v14}[r][r]{1}%
\psfrag{v15}[r][r]{2}%
\psfrag{v16}[r][r]{3}%
\psfrag{v17}[r][r]{4}%
%
% Figure:
\includegraphics[width=\textwidth]{weak_grid4_Sim411.eps.eps}
\end{psfrags}%
%
% End Sim411.eps.tex


==> weak_grid4_Ssp4111v.eps.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{Ssp4111v.eps}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           29-Nov-2010 18:38:45
% eps bounding box:     14.2857 cm x 10.9751 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s04}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$v_{ph}$ [km/s]\end{tabular}}%
\psfrag{s05}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}y [arcsec]\end{tabular}}%
\psfrag{s09}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}log S$_{\lambda}$ [erg/s/cm$^2$/arcsec$^2$/\AA]\end{tabular}}%
%
% xticklabels:
\psfrag{x01}[t][t]{-2000}%
\psfrag{x02}[t][t]{-1500}%
\psfrag{x03}[t][t]{-1000}%
\psfrag{x04}[t][t]{-500}%
\psfrag{x05}[t][t]{0}%
\psfrag{x06}[t][t]{500}%
\psfrag{x07}[t][t]{1000}%
\psfrag{x08}[t][t]{1500}%
\psfrag{x09}[t][t]{2000}%
%
% yticklabels:
\psfrag{v01}[l][l]{-25}%
\psfrag{v02}[l][l]{-24}%
\psfrag{v03}[l][l]{-23}%
\psfrag{v04}[l][l]{-22}%
\psfrag{v05}[l][l]{-21}%
\psfrag{v06}[l][l]{-20}%
\psfrag{v07}[l][l]{-19}%
\psfrag{v08}[l][l]{-18}%
\psfrag{v09}[r][r]{-4}%
\psfrag{v10}[r][r]{-3}%
\psfrag{v11}[r][r]{-2}%
\psfrag{v12}[r][r]{-1}%
\psfrag{v13}[r][r]{0}%
\psfrag{v14}[r][r]{1}%
\psfrag{v15}[r][r]{2}%
\psfrag{v16}[r][r]{3}%
\psfrag{v17}[r][r]{4}%
%
% Figure:
\includegraphics[width=\textwidth]{weak_grid4_Ssp4111v.eps.eps}
\end{psfrags}%
%
% End Ssp4111v.eps.tex


==> weak_grid4_Ssp4112v.eps.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{Ssp4112v.eps}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           29-Nov-2010 18:38:47
% eps bounding box:     14.2857 cm x 10.9751 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s04}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$v_{ph}$ [km/s]\end{tabular}}%
\psfrag{s05}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}z [arcsec]\end{tabular}}%
\psfrag{s09}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}log S$_{\lambda}$ [erg/s/cm$^2$/arcsec$^2$/\AA]\end{tabular}}%
%
% xticklabels:
\psfrag{x01}[t][t]{-2000}%
\psfrag{x02}[t][t]{-1500}%
\psfrag{x03}[t][t]{-1000}%
\psfrag{x04}[t][t]{-500}%
\psfrag{x05}[t][t]{0}%
\psfrag{x06}[t][t]{500}%
\psfrag{x07}[t][t]{1000}%
\psfrag{x08}[t][t]{1500}%
\psfrag{x09}[t][t]{2000}%
%
% yticklabels:
\psfrag{v01}[l][l]{-25}%
\psfrag{v02}[l][l]{-24}%
\psfrag{v03}[l][l]{-23}%
\psfrag{v04}[l][l]{-22}%
\psfrag{v05}[l][l]{-21}%
\psfrag{v06}[l][l]{-20}%
\psfrag{v07}[l][l]{-19}%
\psfrag{v08}[l][l]{-18}%
\psfrag{v09}[r][r]{-4}%
\psfrag{v10}[r][r]{-3}%
\psfrag{v11}[r][r]{-2}%
\psfrag{v12}[r][r]{-1}%
\psfrag{v13}[r][r]{0}%
\psfrag{v14}[r][r]{1}%
\psfrag{v15}[r][r]{2}%
\psfrag{v16}[r][r]{3}%
\psfrag{v17}[r][r]{4}%
%
% Figure:
\includegraphics[width=\textwidth]{weak_grid4_Ssp4112v.eps.eps}
\end{psfrags}%
%
% End Ssp4112v.eps.tex


==> weak_grid7_Nim711.eps.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{Nim711.eps}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           29-Nov-2010 19:48:30
% eps bounding box:     15 cm x 12.5 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s04}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}y [arcsec]\end{tabular}}%
\psfrag{s05}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}z [arcsec]\end{tabular}}%
\psfrag{s06}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Viewpoint: x = -$\infty$\end{tabular}}%
\psfrag{s09}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}log N$_{\textrm{HI}}$   [cm$^{-2}$]\end{tabular}}%
%
% xticklabels:
\psfrag{x01}[t][t]{-8}%
\psfrag{x02}[t][t]{-6}%
\psfrag{x03}[t][t]{-4}%
\psfrag{x04}[t][t]{-2}%
\psfrag{x05}[t][t]{0}%
\psfrag{x06}[t][t]{2}%
\psfrag{x07}[t][t]{4}%
\psfrag{x08}[t][t]{6}%
\psfrag{x09}[t][t]{8}%
%
% yticklabels:
\psfrag{v01}[l][l]{13}%
\psfrag{v02}[l][l]{14}%
\psfrag{v03}[l][l]{15}%
\psfrag{v04}[l][l]{16}%
\psfrag{v05}[l][l]{17}%
\psfrag{v06}[l][l]{18}%
\psfrag{v07}[l][l]{19}%
\psfrag{v08}[l][l]{20}%
\psfrag{v09}[l][l]{21}%
\psfrag{v10}[l][l]{22}%
\psfrag{v11}[l][l]{23}%
\psfrag{v12}[r][r]{-8}%
\psfrag{v13}[r][r]{-6}%
\psfrag{v14}[r][r]{-4}%
\psfrag{v15}[r][r]{-2}%
\psfrag{v16}[r][r]{0}%
\psfrag{v17}[r][r]{2}%
\psfrag{v18}[r][r]{4}%
\psfrag{v19}[r][r]{6}%
\psfrag{v20}[r][r]{8}%
%
% Figure:
\includegraphics[width=\textwidth]{weak_grid7_Nim711.eps.eps}
\end{psfrags}%
%
% End Nim711.eps.tex


==> weak_grid7_Sim711.eps.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{Sim711.eps}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           29-Nov-2010 19:48:36
% eps bounding box:     15 cm x 12.5 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s04}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}y [arcsec]\end{tabular}}%
\psfrag{s05}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}z [arcsec]\end{tabular}}%
\psfrag{s09}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}log S   [erg/s/cm$^2$/arcsec$^2$]\end{tabular}}%
%
% xticklabels:
\psfrag{x01}[t][t]{-8}%
\psfrag{x02}[t][t]{-6}%
\psfrag{x03}[t][t]{-4}%
\psfrag{x04}[t][t]{-2}%
\psfrag{x05}[t][t]{0}%
\psfrag{x06}[t][t]{2}%
\psfrag{x07}[t][t]{4}%
\psfrag{x08}[t][t]{6}%
\psfrag{x09}[t][t]{8}%
%
% yticklabels:
\psfrag{v01}[l][l]{-23}%
\psfrag{v02}[l][l]{-22}%
\psfrag{v03}[l][l]{-21}%
\psfrag{v04}[l][l]{-20}%
\psfrag{v05}[l][l]{-19}%
\psfrag{v06}[l][l]{-18}%
\psfrag{v07}[l][l]{-17}%
\psfrag{v08}[l][l]{-16}%
\psfrag{v09}[r][r]{-8}%
\psfrag{v10}[r][r]{-6}%
\psfrag{v11}[r][r]{-4}%
\psfrag{v12}[r][r]{-2}%
\psfrag{v13}[r][r]{0}%
\psfrag{v14}[r][r]{2}%
\psfrag{v15}[r][r]{4}%
\psfrag{v16}[r][r]{6}%
\psfrag{v17}[r][r]{8}%
%
% Figure:
\includegraphics[width=\textwidth]{weak_grid7_Sim711.eps.eps}
\end{psfrags}%
%
% End Sim711.eps.tex


==> weak_grid7_Ssp7111v.eps.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{Ssp7111v.eps}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           29-Nov-2010 18:41:36
% eps bounding box:     14.2857 cm x 10.9751 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s04}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$v_{ph}$ [km/s]\end{tabular}}%
\psfrag{s05}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}y [arcsec]\end{tabular}}%
\psfrag{s09}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}log S$_{\lambda}$ [erg/s/cm$^2$/arcsec$^2$/\AA]\end{tabular}}%
%
% xticklabels:
\psfrag{x01}[t][t]{-3000}%
\psfrag{x02}[t][t]{-2000}%
\psfrag{x03}[t][t]{-1000}%
\psfrag{x04}[t][t]{0}%
\psfrag{x05}[t][t]{1000}%
\psfrag{x06}[t][t]{2000}%
\psfrag{x07}[t][t]{3000}%
%
% yticklabels:
\psfrag{v01}[l][l]{-25}%
\psfrag{v02}[l][l]{-24}%
\psfrag{v03}[l][l]{-23}%
\psfrag{v04}[l][l]{-22}%
\psfrag{v05}[l][l]{-21}%
\psfrag{v06}[l][l]{-20}%
\psfrag{v07}[l][l]{-19}%
\psfrag{v08}[l][l]{-18}%
\psfrag{v09}[l][l]{-17}%
\psfrag{v10}[r][r]{-8}%
\psfrag{v11}[r][r]{-6}%
\psfrag{v12}[r][r]{-4}%
\psfrag{v13}[r][r]{-2}%
\psfrag{v14}[r][r]{0}%
\psfrag{v15}[r][r]{2}%
\psfrag{v16}[r][r]{4}%
\psfrag{v17}[r][r]{6}%
\psfrag{v18}[r][r]{8}%
%
% Figure:
\includegraphics[width=\textwidth]{weak_grid7_Ssp7111v.eps.eps}
\end{psfrags}%
%
% End Ssp7111v.eps.tex


==> weak_grid7_Ssp7112v.eps.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{Ssp7112v.eps}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           29-Nov-2010 18:41:40
% eps bounding box:     14.2857 cm x 10.9751 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s04}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$v_{ph}$ [km/s]\end{tabular}}%
\psfrag{s05}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}z [arcsec]\end{tabular}}%
\psfrag{s09}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}log S$_{\lambda}$ [erg/s/cm$^2$/arcsec$^2$/\AA]\end{tabular}}%
%
% xticklabels:
\psfrag{x01}[t][t]{-3000}%
\psfrag{x02}[t][t]{-2000}%
\psfrag{x03}[t][t]{-1000}%
\psfrag{x04}[t][t]{0}%
\psfrag{x05}[t][t]{1000}%
\psfrag{x06}[t][t]{2000}%
\psfrag{x07}[t][t]{3000}%
%
% yticklabels:
\psfrag{v01}[l][l]{-25}%
\psfrag{v02}[l][l]{-24}%
\psfrag{v03}[l][l]{-23}%
\psfrag{v04}[l][l]{-22}%
\psfrag{v05}[l][l]{-21}%
\psfrag{v06}[l][l]{-20}%
\psfrag{v07}[l][l]{-19}%
\psfrag{v08}[l][l]{-18}%
\psfrag{v09}[l][l]{-17}%
\psfrag{v10}[r][r]{-8}%
\psfrag{v11}[r][r]{-6}%
\psfrag{v12}[r][r]{-4}%
\psfrag{v13}[r][r]{-2}%
\psfrag{v14}[r][r]{0}%
\psfrag{v15}[r][r]{2}%
\psfrag{v16}[r][r]{4}%
\psfrag{v17}[r][r]{6}%
\psfrag{v18}[r][r]{8}%
%
% Figure:
\includegraphics[width=\textwidth]{weak_grid7_Ssp7112v.eps.eps}
\end{psfrags}%
%
% End Ssp7112v.eps.tex

